Efficient and Private: Memorisation under differentially private parameter-efficient fine-tuning in language models

Fine-tuning large language models (LLMs) for specific tasks introduces privacy risks, as models may inadvertently memorise and leak sensitive training data. While Differential Privacy (DP) offers a solution to mitigate these risks, it introduces significant computational and performance trade-offs, particularly with standard fine-tuning approaches. Previous work has primarily focused on full-parameter updates, which are computationally intensive and may not fully leverage DPs potential in large models. In this work, we address these shortcomings by investigating Parameter-Efficient Fine-Tuning (PEFT) methods under DP constraints. We show that PEFT methods achieve comparable performance to standard fine-tuning while requiring fewer parameters and significantly reducing privacy leakage. Furthermore, we incorporate a data poisoning experiment involving intentional mislabelling to assess model memorisation and directly measure privacy risks. Our findings indicate that PEFT methods not only provide a promising alternative but also serve as a complementary approach for privacy-preserving, resource-efficient fine-tuning of LLMs.

==> tables/dp_setting.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{|l|l|c|c|c|}
\hline
\textbf{Model}      & \textbf{Dataset}    & \textbf{Privacy Budgets (\(\varepsilon\))} & \textbf{Clipping Norm} & \textbf{\(\delta\)}  \\ \hline
DistilBERT          & IMDb, QNLI                & 1.0, 4.0, 8.0                          & 1.5     & 1e-5                   \\ \hline
BERT-base           & IMDb, QNLI          & 4.0                                    & 1.5     & 1e-5                   \\ \hline
\end{tabular}
\caption{Differential Privacy Settings}
\label{table3: DP_settings}
\end{table}
